WetLinks: a Large-Scale Longitudinal Starlink Dataset with Contiguous Weather Data

Low Orbit Satellite (LEO) networks such as Starlink promise Internet access everywhere around the world. In this paper, we present WetLinks - a large and publicly available trace-based dataset of Starlink measurements. The measurements were concurrently collected from two European vantage points over a span of six months. Consisting of approximately 140,000 measurements, the dataset comprises all relevant network parameters such as the upload and download throughputs, the RTT, packet loss, and traceroutes. We further augment the dataset with concurrent data from professional weather stations placed next to both Starlink terminals. Based on our dataset, we analyse Starlink performance, including its susceptibility to weather conditions. We use this to validate our dataset by replicating the results of earlier smaller-scale studies. We release our datasets and all accompanying tooling as open data. To the best of our knowledge, ours is the largest Starlink dataset to date.

==> Acknowledgment.tex <==
% !TEX root = main_ieee.tex

\section{Acknowledgment}\label{sec:ack}
We like to thank Justus Bachmann, Simon Beginn, Alexander Böckenholt, Jan Dunker, Bennet Janzen, and Malte Wehmeier for their help implementing the measurement tools and collecting the data.
This work has been partially supported by the German Federal Ministry for Digital and Transport as part of the “Innovative Network Technologies” funding program (FKZ: 19OI23008C). 


==> Dataset.tex <==
% !TEX root = main_ieee.tex

\section{The SAT-TRAIN Dataset}\label{sec:dataset}
Our measurements in Osnabrück begin on the 14th of September 2023, and in Enschede almost one month later on the 12th of October 2023. Both measurements are planned to be ongoing at least till the end of March 2024. This leads to traces of six and a half months and five and a half months of continuous measurements from Osnabrück and Enschede, respectively.
At the time of publication, the dataset will consist of approx. 80,000 network measurements from Osnabrück, and 60,000 from Enschede.\footnote{A link to the dataset will be added upon acceptance of this paper} 

\subsection{Structural Overview}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Images/FolderStructure.pdf}
    \caption{The file structure of our dataset.}
    \label{fig:file_structure}
\end{figure}

\begin{figure*}
    \centering
    \subfloat[\texttt{net\_iperf.csv}]{
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{lllllll}
            \toprule
            \textbf{timestamp\_start}   
                & \textbf{timestamp\_end}  
                & \textbf{server} 
                & \textbf{ip\_protocol} 
                & \textbf{transport\_protocol} 
                & \textbf{download}
                & \textbf{upload}
                \\ \midrule
            2023-10-12 15:47:42 
                        & 2023-10-12 15:47:43   
                        & 131.173.23.81
                        & v4
                        & UDP
                        & 209647000.0
                        & 16181000.0\\
            2023-10-12 15:47:43     
                        & 2023-10-12 15:4:44
                        & 131.173.23.81
                        & v4
                        & UDP
                        & 167594000.0
                        & 21720000.0\\ \bottomrule
        \end{tabular}
        }
        \label{fig:net_iperf}
    }

    \subfloat[\texttt{net\_ping.csv}]{
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{llllllllll}
            \toprule
            \textbf{timestamp\_start}   
                & \textbf{timestamp\_end}  
                & \textbf{target} 
                & \textbf{ip\_protocol} 
                & \textbf{packet\_loss} 
                & \textbf{packets\_send}      
                & \textbf{ping\_avg}
                & \textbf{ping\_worst}
                & \textbf{ping\_best}
                & \textbf{ping\_stddev}
                
                \\ \midrule
            2023-10-12 15:48:00
                        & 2023-10-12 15:48:49    
                        & 131.173.23.81
                        & v4
                        & 0.0
                        & 250 
                        & 66.425
                        & 128.553
                        & 44.362
                        & 12.458\\
            2023-10-12 15:51:02
                        & 2023-10-12 15:51:51
                        & 131.173.23.81
                        & v4
                        & 0.0
                        & 250
                        & 59.863
                        & 97.087
                        & 47.4
                        & 8.949\\ \bottomrule
        \end{tabular}
        }
        \label{fig:net_ping}
    }

    \subfloat[\texttt{net\_traceroute.csv}]{
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{lllllllllllll}
            \toprule
            \textbf{timestamp\_start}   
                & \textbf{timestamp\_end}  
                & \textbf{hop}
                & \textbf{target} 
                & \textbf{ip\_protocol} 
                & \textbf{hop\_id}
                & \textbf{asn}
                & \textbf{packet\_loss} 
                & \textbf{packets\_send}      
                & \textbf{ping\_avg}
                & \textbf{ping\_worst}
                & \textbf{ping\_best}
                & \textbf{ping\_stddev}
                
                \\ \midrule
            2023-10-12 15:51:53
                        & 2023-10-12 15:52:14
                        & 1
                        & 131.173.23.81
                        & v4
                        & \_gateway (10.13.37.254)
                        & AS???
                        & 0.0
                        & 15 
                        & 0.22
                        & 0.27
                        & 0.18
                        & 0.04\\
            2023-10-12 15:51:53
                        & 2023-10-12 15:52:14
                        & 2
                        & 131.173.23.81
                        & v4
                        & 100.64.0.1
                        & AS???
                        & 0.0
                        & 15
                        & 45.62
                        & 55.64
                        & 33.67
                        & 7.04\\ \bottomrule
        \end{tabular}
        }
        \label{fig:net_traceroute}
    }

    \subfloat[\texttt{starlink.csv}]{
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{lllllllllllllll}
            \toprule
            \textbf{timestamp}   
                & \textbf{state}  
                & \textbf{uplink}
                & \textbf{downlink} 
                & \textbf{pop\_ping\_latency} 
                & \textbf{ping\_drop}
                & \textbf{mean\_ping\_latency}
                & \textbf{ping\_stdvar} 
                & \textbf{fraction\_obstructed}      
                & \textbf{obstruction\_duration}
                & \textbf{obstruction\_interval}
                & \textbf{direction\_azimuth}
                & \textbf{direction\_elevation}
                & \textbf{lat}
                & \textbf{lon}
                
                \\ \midrule
            2023-10-12 15:47:01
                        & CONNECTED
                        & 3447.72
                        & 8858.37
                        & 28.9524
                        & 0.1929
                        & 33.5903
                        & 15.9871
                        & 0.0
                        & 0.0
                        & 0.0
                        & 179.239
                        & 70.3973
                        &
                        & \\
            2023-10-12 15:48:02
                        & CONNECTED
                        & 41557.2
                        & 31306.3
                        & 45.9
                        & 0.2929
                        & 32.9442
                        & 15.8419
                        & 0.0
                        & 0.0
                        & 0.0
                        & 179.133
                        & 70.0242
                        & 
                        & \\ \bottomrule
        \end{tabular}
        }
        \label{fig:starlink}
    }

    \subfloat[\texttt{froggit.csv}]{
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{llllllllllllllllll}
            \toprule
            \textbf{timestamp}   
                & \textbf{temp}  
                & \textbf{humidity}
                & \textbf{dewpt} 
                & \textbf{windchill} 
                & \textbf{winddir}
                & \textbf{windspeed}
                & \textbf{windgust} 
                & \textbf{rain}      
                & \textbf{rain\_daily}
                & \textbf{rain\_weekly}
                & \textbf{rain\_monthly}
                & \textbf{rain\_yearly}
                & \textbf{solarradiation}
                & \textbf{uv}
                & \textbf{barom}
                & \textbf{lowbatt}
                & \textbf{softwaretype}
                
                \\ \midrule
            2023-10-12 15:47:25
                        & 15.0
                        & 98
                        & 14.7
                        & 15.0
                        & 0
                        & 1.998
                        & 2.298
                        & 1.8034
                        & 17.5006
                        & 21.7932
                        & 28.6004
                        & 63.5
                        & 67.09
                        & 0
                        & 1007.69
                        & 0 
                        & GW2000A\_V2.2.4\\
            2023-10-12 15:48:26
                        & 15.1
                        & 98
                        & 14.8
                        & 15.1
                        & 17
                        & 1.4
                        & 2.298
                        & 1.1938
                        & 17.5006
                        & 21.7932
                        & 28.6004
                        & 63.5
                        & 59.91
                        & 0
                        & 1007.79
                        & 0
                        & GW2000A\_V2.2.4 \\ \bottomrule
        \end{tabular}
        }
        \label{fig:froggit}
    }
    \caption{Overview of the different \texttt{.csv} files forming our dataset.}
    \label{fig:dataset_overview}
\end{figure*}

The dataset consists of multiple \texttt{.csv} files containing the main data. Each of these files has an accompanying \texttt{.txt} file that describes the format of each feature of the \texttt{.csv}. We provide separate files for the measurements in Osnabrück and Enschede. Fig. \ref{fig:file_structure} provides an overview of the file structure. Fig. \ref{fig:dataset_overview} gives an overview of the data in the \texttt{.csv} files. The main dataset is provided in the \texttt{net\_iperf.csv}, \texttt{net\_ping.csv}, \texttt{net\_traceroute.csv}, \texttt{starlink.csv}, and \texttt{froggit.csv}.

\texttt{net\_iperf.csv} contains the throughput measurements. One row contains the \textit{iperf3} measurement result of one second. Consequently, 15 rows can be aggregated to form one measurement point. In addition to the download and upload speed in bits/s, the used transport protocol, the IP version, the IP of the server, and a start and end timestamp in ISO8601 format are included.

\texttt{net\_ping.csv} contains the results for the latency measurements. Each entry consists of a start and end timestamp, the IP address of the target server, the IP version that is used (here, IPv4), the packet loss rate in percent, the total number of ICMP packets that have been sent for this measurement, and the average-, worst-, and best ping, as well as the standard deviation of the total number of ICMP packets sent.

\texttt{net\_traceroute.csv} contains the mtr results. One mtr measurement consists of multiple rows, as each single row corresponds to one hop of a measurement. All rows belonging to one measurement share the same start and end timestamps. In addition, the hop counter, the target IP address, the IP version, the hop\_id, the Autonomous System Number (asn), the packet loss rate, the total number of packets sent for this measurement, and the ping statistics of this measurement (average, worst, best, standard deviation) are included for every row.

\texttt{starlink.csv} contains the data that is automatically collected by the dish and periodically requested by our scripts. This includes the timestamp, a state indicating if the dish is connected, the uplink and downlink throughputs in Mbit/s, the pop ping latency, the dropped pings in \%, the average ping latency, the ping standard deviation, the portion of the dish that is obstructed in \%, the duration of the obstruction in s, the obstruction interval in s, the direction azimuth in degrees celsius, the direction elevation in degrees celsius, and the latitude and longitude of the dish.

\texttt{froggit.csv} contains the weather data collected by the Froggit DP2000 weather station placed directly next to the dish. One entry consists of the features listed in Tables \ref{tab:froggit_features} and \ref{tab:froggit_calculated_features}. In addition, a low battery field indicating the battery status (0 = OK, 1 = Low), and the current firmware version are included.

In addition to this main dataset, we also provide important measurement metadata in the \texttt{metadata.csv}. These include, for example, detailed system information of our measurement system, version information of all libraries and tools that we used, as well as hardware information about our Starlink dishes.

\subsection{Preprocessing}
We provide the dataset in unfiltered raw format. Similar to most available datasets, we also recommend certain preprocessing steps in order to use our dataset.

First, \texttt{net\_iperf.csv} contains the raw output of the \texttt{iperf3} measurement tool. During one measurement, \texttt{iperf3} outputs intermediate results for every second of the measurement. This means that one row of our dataset represents one of these intermediate results.
We recommend aggregating them by calculating the mean to get aggregated values for the download and upload throughputs to represent one measurement.

Second, as described in Sec.~\ref{sec:setup}, different sensors have different measurement frequencies.
For example, the weather is measured in smaller time intervals than the network parameters.
If these parameters should be analyzed together, we recommend aggregating the higher-frequency ones to the same measurement intervals as the network parameters. This can be done by searching the $k$ closest measurements of the higher frequency parameter to every network parameter measurement based on the timestamps and calculating the means. 
For example, for our analysis of the weather impact on the network parameters (cf. Sec.~\ref{sec:analysis:weather}), we calculated the means of the nearest three weather measurements for every network parameter measurement.

We provide scripts for all of the preprocessing steps, as well as the scripts for our analysis, to ensure full replicability of our results.

\subsection{Limitations}
Our dataset has a few minor limitations that are automatically handled by our preprocessing scripts.

First, some measurements in the \texttt{net\_iperf.csv} may have empty fields for the download and/or upload column. This occurs rarely and is caused by an error in the \textit{iperf} start-up or by an error during the \textit{iperf} run. The resulting empty fields are usually interpreted as \textit{NAN} values by most data analysis tools like pandas\footnote{\url{https://pandas.pydata.org}} and can be filtered out.

Second, \texttt{net\_traceroute.csv} contains measurements with only two hops and very high RTTs around 1s at the second hop. This may be caused by short Starlink outages or erroneous runs of mtr. This happens very rarely and only affects approx. less than 10 measurements at both measurement sites. These measurements can be filtered out based on the hop count.

Third, the Froggit weather station in Enschede had a downtime of approximately two weeks in December 2023 / January 2024 due to an empty battery. While the network measurements were running, there is no weather data available for this time-span.

%\subsection{Usage Scenarios}
%We created this dataset primarily with the ongoing rise of ML-based solutions for many networking problems in mind.
%Our primary use-case is rate-adaptation for video streaming \cite{zhou2021vibra}, 360° video streaming \cite{kan2021rapt360}, DASH-like point cloud streaming \cite{zhang2022trans}, and real-time point cloud streaming for robotic applications \cite{laniewski2021potential}.
%The solutions in these areas are typically based on deep reinforcement learning (DRL) algorithms, which require varying network conditions to avoid overfitting.

%Nonetheless, the usage of our dataset is not limited to these areas. It could be used for any use-case where traces of real-world measurements of Satellite networks are useful. Interesting areas could be, for example, agricultural robotics where sensor data needs to be transmitted in real-time from places where no 4G or 5G coverage exists.

